Loewner-based Data-driven Iterative Structured Control Design

Stability enforcement remains a challenge in data-driven control paradigms, where no parametrised model of the system is available. For instance, the system's instabilities can be estimated in order to enforce a closed-loop stability constraint on the controller reduction step. In order to avoid this preliminary estimation of instabilities, this paper proposes to embed a closed-loop stability constraint in the design. To that extent, an optimization problem is formulated in order to improve matching between the reference model and the closed-loop while maintaining internal stability. The proposed iterative procedure to solve this problem is illustrated on two numerical examples.

==> rebut.tex <==
The objective of the next sections is to specify the internal stability criterion, the chosen objective norm and the chosen controller structure to provide a implementable version of the problem $\mathcal{P}$ \eqref{P}. To make the problem easier to solve, it has been preferred to consider only sufficient criterion for internal stability based on the knowledge of an initial internally stabilizing controller. %Nevertheless, since the obtained controller leads to internal stability as well, one may consider the opportunity to use it as a new initial controller and iterate the process to enlarge the research space.



\subsection{Adaptation of the method for PI and PID controller}
As popular control structure such as PI and PID $\notin \mathcal{RH}_\infty$, the method must be adapted to account for these cases.

Let us suppose that the desired controller form does not belong to $\mathcal{RH}_\infty$. Let us also suppose that a controller with the desired form, leading to internal stability $\mathbf{K}_0$ is available. Then it is possible to find a transfer $\mathbf{F}$ such that
\begin{equation}
\begin{array}{c}
     \Tilde{\mathbf{K}}_0=\mathbf{F}\mathbf{K}_0 \\
     \Tilde{\mathbf{K}}(\theta)=\mathbf{F}\mathbf{K}(\theta)
\end{array},
\end{equation}
where $\Tilde{\mathbf{K}}_0 \in \mathcal{RH}_\infty$ and $\Tilde{\mathbf{K}}(\theta) \in \mathcal{RH}_\infty$.

\begin{figure}
    \centering
    \scalebox{0.8}{\begin{tikzpicture}[auto, node distance=1cm]
    \node [input, name=input] {r};
    \node[sum, right of=input,node distance=0.5cm](sum1){};
    \node[temporaire, right of=sum1,node distance=0.5cm](tempo1){};
    \node[block, right of=tempo1](controller_1){$\mathbf{K}_0$};
    \node[block, above of=controller_1,node distance=1cm](controller_2){$\Tilde{\mathbf{K}}_1-\Tilde{\mathbf{K}}_0$};
    \node[sum, right of=controller_1,node distance=1.5cm](sum2){};
    \node[block, right of=sum2,node distance=1.25cm](filter){$\mathbf{F}^{-1}$};
    \node[block, right of=filter, node distance=2cm](plant){$\mathbf{P}$};
    \node[temporaire, below of=controller_1,node distance=1cm](tempo2){};
    \node[temporaire, right of=plant,node distance=1cm](tempo3){};
    \node[output, name=output,right of=plant,node distance=1.25cm]{};
    
    \draw[->] (input)--node[name=r,pos=0.60]{$r$\quad $+$}(sum1);
    \draw[-] (sum1)--node[name=epsilon]{$\epsilon$}(tempo1);
    \draw[->](tempo1)--(controller_1);
    \draw[->](tempo1)|-(controller_2);
    \draw[->](controller_1)--node[name=command_1,pos=0.3]{$u_0$}node[name=plus1,pos=0.9]{+}(sum2);
    \draw[->](controller_2)-|node[name=command_2,pos=0.2]{$\Tilde{u_1}$}node[name=plus2,pos=0.9]{+}(sum2);
    \draw[->] (sum2)--(filter);
    \draw[->](filter)--node[name=command]{$u_1$}(plant);
    \draw[->](plant)--node[name=tempo4]{$y$}(output);
    \draw[-](tempo3)|-(tempo2);
    \draw[->](tempo2)-|node[name=moins,pos=0.9]{-}(sum1);
    \end{tikzpicture}}
    \caption{non-$\mathcal{RH}_\infty$ controller interconnection}
    \label{fig:non RHinf controller incterconnection}
\end{figure}

Then the interconnection in Figure \ref{fig:Small gain interconnection} can be replaced by the interconnection in Figure \ref{fig:non RHinf controller incterconnection}. It is then possible to merge the transfer $\mathbf{F}^{-1}$ and $\mathbf{P}$ to compute a new plant data $\Tilde{\Phi}_k$ such that
\begin{equation}
\begin{array}{cc}
    \Tilde{\Phi}_k=\Phi_k\mathbf{F}(\imath\omega_k)^{-1}& 1\leq k\leq N.
\end{array}
\end{equation}
Then, the same optimization problem $\mathcal{P}_1$ \eqref{P3} can be formulated with $\Tilde{\mathbf{K}}_0$ instead of $\mathbf{K}_0$, $\Tilde{\mathbf{K}}(\theta)$ instead of $\mathbf{K}(\theta)$, $\Tilde{\Phi}_k$ instead of $\Phi_k$ and $\Tilde{\gamma}_0$ instead of$\gamma_0$.


For instance, for a PID controller, $\mathbf{K}(s)=k_P+\frac{k_I}{s}+\frac{k_D s}{1+\tau s}$, $\mathbf{F}$ can be chosen as $\mathbf{F}(s)=\frac{s}{s+a}$, with $a$ a real positive number to avoid instabilities. With this transfer,

\begin{equation}
    \begin{array}{cc}
         \Tilde{\mathbf{K}}(s)=\frac{(k_p\tau+k_d)s^2+(k_p+k_i\tau)s+k_i}{(s+a)(1+\tau s)}& \in\mathcal{RH}_\infty \\

            \Tilde{\Phi}_k=\Phi_k\cdot\frac{\imath\omega_k+a}{\imath\omega_k} & 1\leq k\leq N  
    \end{array}
\end{equation}

\begin{figure}
    \centering
    \subfloat{
    \begin{tikzpicture}
    \node[] {\includegraphics[width=0.23\textwidth]{figures/Freq_resp_f16_11_NB.pdf}};
    \draw (0,1.4) node[above]{\textcolor{blue}{$r_{ref}$} $\delta_a$};
    \draw (-2.3,0) node[] {$r$};
    %\draw (-2.3,0) node[below] {$\delta_a$};
    \end{tikzpicture}}
    \hspace*{-0.8cm}
    \subfloat{
    \begin{tikzpicture}
    \node[] {\includegraphics[width=0.23\textwidth]{figures/Freq_resp_f16_12_NB.pdf}};
    \draw (0,1.4) node[above]{\textcolor{blue}{$y_{ref}$} $\delta_r$};
    \end{tikzpicture}}
    \vspace*{-0.95cm}\\
    \subfloat{
    \begin{tikzpicture}
    \node[] {\includegraphics[width=0.23\textwidth]{figures/Freq_resp_f16_21_NB.pdf}};
    \draw (-2.3,0) node[] {$y$};
    %\draw (-2.3,0) node[below] {$\delta_r$};
    \end{tikzpicture}}
    \hspace*{-0.8cm}
    \subfloat{
    \begin{tikzpicture}
    \node[] {\includegraphics[width=0.23\textwidth]{figures/Freq_resp_f16_22_NB.pdf}};
    \end{tikzpicture}
    }
    \vspace*{-0.3cm}  
    \caption{Frequency response of the angle control}
    \vspace*{-0.3cm}
    \label{fig:Frequency response of the angle control f16 air_fighter}
    \end{figure}
    
    
    %\subfloat{
    \includegraphics[width=0.49\linewidth]{figures/Freq_resp_f16_11_NB.pdf}
    %}
    %\subfloat{
    \includegraphics[width=0.49\linewidth]{figures/Freq_resp_f16_12_NB.pdf}
    %}
    %\subfloat{
    \includegraphics[width=0.49\linewidth]{figures/Freq_resp_f16_21_NB.pdf}
    %}
    %\subfloat{
    \includegraphics[width=0.49\linewidth]{figures/Freq_resp_f16_22_NB.pdf}
    %}
